Stacking the spectra of eROSITA galaxy cluster data for searches of the 3.5keV line: Dark matter decay or charge exchange?

In this Master Thesis, we use a technique to shift and stack the X-Ray spectra of 1138 galaxy clusters from the eRASS-1 survey, totalling 430649 counts. In comparison with previous stacking techniques, the method presented here introduces proper normalization of the shifted redistribution matrix file (RMF), which allows to recover the physical temperature and metallicity of the stacked spectra. Using this technique, we can obtain constraints in the stacked spectra for the individual abundances of O, Ne, Mg, Si, Ar, Ca, and Fe. Additionally, we study the possible detection of the previously reported 3.5keV unidentified line emission; however, the residuals barely exceed $\pm 2 \sigma$ in the [3-4]keV range. On the other hand, although residuals in the [3.4-3.55]keV band are compatible with charge exchange emission from SXVI (bare sulphur ions), charge exchange emission from OVII at 0.56keV should also be present, since it is 200 orders of magnitude higher than charge emission from SXVI in the [3.4-3.55]keV band; however, it is unfortunately not detected.

==> Abstract.tex <==
\addcontentsline{toc}{chapter}{\protect Abstract}
\chapter*{Abstract}

% This is the abstract

==> Acknowledgements.tex <==
\addcontentsline{toc}{chapter}{\protect Acknowledgements}
\chapter*{Acknowledgements}
\thispagestyle{empty}
